Black-box Model Ensembling for Textual and Visual Question Answering via Information Fusion

A diverse range of large language models (LLMs), e.g., ChatGPT, and visual question answering (VQA) models, e.g., BLIP, have been developed for solving textual and visual question answering tasks. However, fine-tuning these models is either difficult, as it requires access via APIs, rendering them as black-boxes, or costly due to the need of tuning a large number of parameters. To address this, we introduce InfoSel, a data-efficient ensemble method that learns to dynamically pick the winner from existing black-box models for predictions on both textual and multimodal visual question answering tasks. Unlike traditional ensemble models, InfoSel does not rely on prediction probabilities or confidences, which typically are not available in black-box models. Experimental results on four datasets demonstrate that our approach achieves an absolute increase of up to +5.19\% in the F1-score compared to standalone LLMs using only 1K training instances.

==> abstract.tex <==

A diverse range of large language models (LLMs), e.g., ChatGPT, and visual question answering (VQA) models, e.g., BLIP, have been developed for solving textual and visual question answering tasks. However, fine-tuning these models is either difficult, as it requires access via APIs, rendering them as black-boxes, or costly due to the need of tuning a large number of parameters. To address this, we introduce \textbf{\ourname}, a data-efficient ensemble method that learns to dynamically pick the winner from existing black-box models for predictions on both textual and multimodal visual question answering tasks. Unlike traditional ensemble models, \textbf{\ourname} does not rely on prediction probabilities or confidences, which typically are not available in black-box models. 
Experimental results on four datasets demonstrate 
that our approach achieves an absolute increase of up to +5.19\% in the F1-score compared to standalone LLMs using only 1K training instances. 
% Remarkably, this improvement is achieved by utilizing only 1K training instances and 110M model parameters for training task-specific ensemble models.

% (Klim) To tackle this issue of fine-tuning on task-specific datasets... we propose ensemble.... Unlike existing ensemble techniques, our approach allows to .... <<work without scoring>>..... Furthermore, our proposed method is designed to work with limited training data....

% The latest ensemble techniques as a compelling alternative taking the prediction confidences as part of the inputs are also not applicable as LLMs do not provide confidences. 
% Under the constraints of limited computing and labeled data resources as well as a lack of prediction confidence, we introduce a new data-efficient ensemble method named \textbf{\ourname}, which trains an ensemble model to select the best answer from the predictions of existing black-box models without relying on confidence scores for both textual and visual question answering tasks. 


% Our results demonstrate that training an \textbf{\ourname}-BERT model (only $1/1750 $ of parameters than ChatGPT) increases up to 5.27\% F1-score using less than 0.8\% of training data on SQuAD-V2. 


% Similar improvements showed on NQ-Open, GQA, VizWiz.

% A variety of pre-trained models with different architectures for Visual Question Answering (VQA) tasks have been developed and trained on standard datasets.
% However, these models can have difficulty generalizing to new domains. 
% Fine-tuning on data of the new domain, in order to improve the generalization of the model, is restricted to \emph{white-box} models, where model weights are accessible and not hidden via a service or an API. 
% Additionally, fine-tuning can be computationally expensive due to the large model size. 
% Ensemble methods like majority voting, on the other hand, can combine the predictions of pre-trained models
% even in cases where model weights are not accessible (\emph{black-box} models) with low computational costs. In this work, we aim to improve performance on new domains by leveraging existing VQA models trained on VQA v2 in  \emph{black-box}  settings with limited development data.
% We propose \ourname, which is a new sample-specific  ensemble method that trains an ensemble model with low computational cost to select the best answer for different inputs. Our results demonstrate that  \ourname   \/ improves out-domain performance on GQA (50.60\% to 55.29\%) and VizWiz (32.85\% to 42.06\%).

% (add specific numbers, not mentioning datasets too much)
% For the \emph{white-box} setting, we compare the performance of \ourname{} to fine-tuning and find that ensemble does not provide an additional advantage.


==> cover_letter.tex <==
\item Dear Dr. Salvador García-Lopez,,

\item We are pleased to submit our manuscript entitled “Information Fusion for Black-box Textual and Visual Question
Answering Ensembling” for your consideration at The Journal of Information Fusion. Our paper presents \ourname, an efficient black-box ensemble method that dynamically selects optimal predictions from large language models (LLMs) and visual question answering (VQA) models, addressing limitations in tuning and model accessibility by treating these models as “black-boxes.”

\item Our research aligns closely with the mission of The Journal of Information Fusion to promote advancements in data and decision fusion across diverse applications. \ourname\ achieves significant gains on both textual and multimodal question-answering tasks without requiring fine-tuning or prediction confidences, making it particularly valuable in settings where models are only accessible via APIs and cannot be modified or retrained. This characteristic directly supports the journal’s focus on multi-source information fusion by leveraging diverse models in a coherent, dynamically adaptive ensemble system that advances the fields of natural language processing and multimodal fusion.

\item Our approach is unique compared to traditional ensemble methods, which typically rely on probabilistic outputs unavailable in black-box settings. Instead, \ourname\ uses a data-efficient training approach to learn optimal model selection patterns, achieving performance gains of up to +5.19\% in F1-score with as few as 1,000 training examples across four standard datasets. We believe that this research has broad applications, including in real-time decision-making, AI-driven question answering, and multimodal content understanding, and aligns with the journal’s emphasis on practical, real-world fusion applications in fields like AI, robotics, and automated systems.

\item We believe that The Journal of Information Fusion is an ideal venue for our work, as it will reach researchers focused on information fusion across textual, visual, and multimodal domains. We confirm that this manuscript is original, has not been published elsewhere, and is not under consideration by any other journal. All authors have approved the manuscript, and there are no conflicts of interest to declare.

\item Thank you for considering our submission. We look forward to the opportunity to contribute to The Journal of Information Fusion and share our findings with its readership. Please do not hesitate to contact us should you require further information.

\item  Sincerely,
[Your Full Name]
[Your Position/Title]
[Your Institution/Organization]



==> tables/case_study_table_merged.tex <==


\begin{subtable}[b]{0.45\linewidth} % Adjusted width to fit within the page
    \centering
    \caption{{\normalsize Textual Question Answering}}
    \noalign{\vskip 0.5cm}
    % Your content here (table, text, or figures)
\addtolength{\tabcolsep}{-0.1em} % cut of hlines from the right

\begin{tabular}{|l|cc|}

 \hline

 &  \textbf{Mini-SDv2} & \textbf{Mini-NQ}  \\
 
 \textbf{} &  ... Derrick Norman   &  ... in 2005 and the \\
  \textbf{Context:} & Lehmer's list   &   release of her epon- \\
  \textbf{} & of primes up to    &   ymous debut album\\
 \textbf{} &  10,006,721 ...  &  the following year ...\\
  \hline
 \textbf{} &  How many primes were & When did Taylor  \\
 \textbf{Question:} &   included in Derrick  &  Swift 's first \\
  \textbf{} &  Norman Lehmer's list    &  album release?\\
   \textbf{} &  of prime numbers?  & \\
\hline

 % U-VisualBERT &51.53& 45.02&&\\
LLaMA  & unanswerable & 2006\\
Davinci &  \textbf{10,006,721} &  2006\\
ChatGPT & unanswerable &2006\\
\hline
FT-BERT & unanswerable  &\textbf{\textcolor{red}{2005}}\\
\textbf{\ourname-TT} & \textbf{10,006,721} &  {2006}\\
\textbf{\ournameplus-TT} &unanswerable & \textbf{\textcolor{red}{2005}}\\
\hline

\end{tabular}

\end{subtable}
&
% Subtable 2
\begin{subtable}[b]{0.48\linewidth} % Adjusted width to fit within the page
    \centering
    \caption{\normalsize Visual Question Answering}
    \noalign{\vskip 0.5cm}
    % Your content here (table, text, or figures)
    \begin{tabular}{|l|cc|}
\hline
 &  \textbf{Mini-GQA} &  \textbf{Mini-Viz} \\
 
{\textbf{Image:}} & \includegraphics[width=0.28\linewidth, height=18mm]{images/n314630.jpg} & \includegraphics[width=0.28\linewidth, height=18mm]{images/VizWiz_val_00003469.jpg}\\

 \textbf{Question:} & What appliance is    & What is this pro-  \\

 
 \textbf{} & it?&  duct?\\
\hline

ALBEF &blender&  refrigerator\\
BLIP  & \textbf{toaster} & toilet\\
VLMo &microwave & door\\
\hline
FT-MT & coffee maker & \textbf{unanswerable}\\
\textbf{\ourname-MT} & \textbf{toaster} & toilet\\
\textbf{\ournameplus-MT} & coffee maker & \textbf{unanswerable}\\

\hline

\end{tabular}

\end{subtable}




% \begin{subtable}{0.4\textwidth}
% \centering
% \caption{Textual Question Answering}

% \addtolength{\tabcolsep}{-0.1em} % cut of hlines from the right

% \begin{tabular}{l|cc}
% \hline

%  &  \textbf{Mini-SDv2} & \textbf{Mini-NQ}  \\
 
%  \textbf{} &  ... Derrick Norman   &  ... in 2005 and the \\
%   \textbf{Context:} & Lehmer's list   &   release of her epon- \\
%   \textbf{} & of primes up to    &   ymous debut album\\
%  \textbf{} &  10,006,721 ...  &  the following year ...\\
%   \hline
%  \textbf{} &  How many primes were & When did Taylor  \\
%  \textbf{Question:} &   included in Derrick  &  Swift 's first \\
%   \textbf{} &  Norman Lehmer's list    &  album release?\\
%    \textbf{} &  of prime numbers?  & \\
% \hline

%  % U-VisualBERT &51.53& 45.02&&\\
% LLaMA  & unanswerable & 2006\\
% Davinci &  \textbf{10,006,721} &  2006\\
% ChatGPT & unanswerable &2006\\
% \hline
% FT-BERT & unanswerable  &\textbf{\textcolor{red}{2005}}\\
% \textbf{\ourname-TT} & \textbf{10,006,721} &  {2006}\\
% \textbf{\ournameplus-TT} &unanswerable & \textbf{\textcolor{red}{2005}}\\
% \hline

% \end{tabular}

% \end{subtable}

% &
% % \hspace{1.1cm}

% \begin{subtable}{0.42\textwidth}
% \centering
% \caption{Visual Question Answering}
% % \footnotesize
% \addtolength{\tabcolsep}{-0.1em} % cut of hlines from

% \begin{tabular}{l|cc}
% \hline
%  &  \textbf{Mini-GQA} &  \textbf{Mini-Viz} \\
 
% {\textbf{Image:}} & \includegraphics[width=0.28\linewidth, height=20mm]{images/n314630.jpg} & \includegraphics[width=0.28\linewidth, height=20mm]{images/VizWiz_val_00003469.jpg}\\

%  \textbf{Question:} & What appliance is    & What is this pro-  \\

 
%  \textbf{} & it?&  duct?\\
% \hline

% ALBEF &blender&  refrigerator\\
% BLIP  & \textbf{toaster} & toilet\\
% VLMo &microwave & door\\
% \hline
% FT-MT & coffee maker & \textbf{unanswerable}\\
% \textbf{\ourname-MT} & \textbf{toaster} & toilet\\
% \textbf{\ournameplus-MT} & coffee maker & \textbf{unanswerable}\\

% \hline

% \end{tabular}

% \end{subtable}

==> tables/llm_main_full_table.tex <==


\begin{tabular}{l|llll|llll}
\hline
&\multicolumn{4}{c}{\textbf{SQuAD-V2}} & \multicolumn{4}{c}{\textbf{NQ-Open}}\\
% \textbf{Model} &  \multicolumn{1}{c}{\textbf{Val}} & \multicolumn{1}{c}{\textbf{Test} }& \multicolumn{2}{c}{\textbf{Val}}& \multicolumn{1}{c}{\textbf{Test}}\\

\cline{2-9}
\textbf{} & \textbf{EM} & \textbf{P} & \textbf{R} &\textbf{F1}& \textbf{EM} & \textbf{P} & \textbf{R} &\textbf{F1} \\
\hline

% FLAN-T5-XXL&74.79 & 83.71 & 83.74 & 82.48&&&&\\
LLaMA-2-70b& 0.24 & 7.20 & 52.7 & 11.34    & 28.07 & 43.20 & 79.21 & 46.47\\
Davinci-003& 52.37 & 56.86 & 63.58 & 58.44 &52.24 & 69.96 & 77.50 & 69.44\\
ChatGPT &	30.89 & 40.53 & 68.54 & 44.95  &57.53 & 74.15 & 75.81 & 71.54\\
\textbf{Oracle} & 58.61 & 64.04 & 77.98 & 66.20& 64.02 & 80.54 & 87.97 & 79.21\\
\hline
MV & 26.95 & 34.23 & 61.22 & 37.75 & 46.07 & 62.56 & 77.66 & 62.43\\
WV  & 52.37 & 56.86 & 63.58 & 58.44  & 57.53 & 74.15 & 75.81 & 71.54\\
% Q-Cluster  &56.10 & 51.18&&\\
% QI-Cluster  & 56.38& 51.20&&\\
% \ourname-MLP &57.87&52.35&22.68&18.75&21.12\\
% $Selector_s$&58.21 &47.52&& \\
\hline
FT-BERT 10 & 27.22 & 28.2 & 30.13 & 28.47& 3.92 & 11.05 & 18.49 & 11.23\\
FT-BERT 20 & 47.89 & 47.95 & 48.11 & 47.98&  6.89 & 14.74 & 21.71 & 14.44\\
FT-BERT 40 & 49.98 & 49.95 & 49.95 & 49.95& 10.75 & 19.32 & 22.36 & 17.47\\
FT-BERT 60 & 50.1 & 50.07 & 50.07 & 50.07& 12.03 & 20.8 & 23.33 & 18.9\\
FT-BERT 80 & 50.1 & 50.07 & 50.07 & 50.07&  16.03 & 23.53 & 23.6 & 21.0\\
FT-BERT 100 &50.1 & 50.07 & 50.07 & 50.07&  17.78 & 24.6 & 23.88 & 22.07\\
FT-BERT 300 & 47.45 & 47.86 & 48.67 & 47.96& 24.15 & 29.37 & 29.64 & 27.4\\
FT-BERT 600 & 42.41 & 43.15 & 44.51 & 43.22& 32.18 & 38.83 & 39.53 & 36.55 \\
FT-BERT 1000 & 46.8 & 47.7 & 48.86 & 47.68& 36.52 & 42.81 & 43.46 & 40.6\\
FT-BERT 2000 & 49.71 & 50.64 & 51.91 & 50.65& 43.04 & 49.29 & 49.06 & 46.78\\
FT-BERT 4000 & 52.1 & 53.84 & 55.62 & 53.89&  48.59 & 55.2 & 54.21 & 52.23\\
FT-BERT 6000 & 55.48 & 56.94 & 58.18 & 56.82& 51.93 & 58.25 & 56.52 & 54.92\\
FT-BERT 8000 & 54.88 & 56.27 & 57.84 & 56.35& 51.73 & 58.9 & 56.68 & 55.15\\
FT-BERT 10000 &56.96 & 58.34 & 59.85 & 58.31& 53.82 & 59.86 & 57.91 & 56.38\\
FT-BERT 12000 & 57.85 & 59.1 & 60.1 & 58.96&  54.67 & 60.49 & 58.3 & 57.0\\
FT-BERT 14000 & 58.75 & 59.85 & 60.88 & 59.73& 53.44 & 59.29 & 56.71 & 55.74\\
FT-BERT 16000 &58.49 & 59.68 & 60.56 & 59.49&  55.62 & 61.41 & 59.16 & 58.05\\
FT-BERT 18000 & 58.77 & 59.87 & 60.91 & 59.79& 55.76 & 61.66 & 59.38 & 58.11\\
\textbf{\ourname-BERT 10} & 51.83 & 56.36 & 63.74 & 61.78& 56.19 & 73.66 & 74.22 & 70.41\\
\textbf{\ourname-BERT 20} & 52.25 & 56.67 & 63.7 & 63.03&  56.36 & 73.91 & 74.03 & 70.64\\
\textbf{\ourname-BERT 40} & 52.35 & 56.83 & 63.59 & 63.44& 57.3 & 74.93 & 74.8 & 71.5\\
\textbf{\ourname-BERT 60} & 52.24 & 56.74 & 63.62 & 63.2& 53.33 & 71.0 & 76.19 & 68.54\\
\textbf{\ourname-BERT 80} & 52.36 & 56.81 & 63.57 & 63.02&  56.56 & 74.05 & 75.65 & 70.93\\
\textbf{\ourname-BERT 100} &52.34 & 56.84 & 63.58 & 63.57&  56.67 & 73.81 & 75.18 & 71.03\\
\textbf{\ourname-BERT 300}  & 52.35 & 56.85 & 63.59 & 63.63&  57.93 & 74.87 & 75.85 & 71.91\\
\textbf{\ourname-BERT 600}  & 52.35 & 56.84 & 63.56 & 63.29&  58.3 & 75.75 & 76.53 & 72.74\\
\textbf{\ourname-BERT 1000} & 52.36 & 56.85 & 63.59 & 63.71&  58.45 & 75.99 & 77.75 & 73.37\\
\textbf{\ourname-BERT 2000} & 52.33 & 56.84 & 63.62 & 63.58&  58.96 & 76.25 & 77.31 & 73.39\\
\textbf{\ourname-BERT 4000} & 52.35 & 56.85 & 63.58 & 63.63&  59.3 & 76.8 & 77.96 & 73.85\\
\textbf{\ourname-BERT 6000} & 52.34 & 56.84 & 63.62 & 63.67&  59.59 & 76.62 & 78.15 & 73.91\\
\textbf{\ourname-BERT 8000} & 52.33 & 56.82 & 63.61 & 63.42&  59.25 & 76.44 & 77.75 & 73.6\\
\textbf{\ourname-BERT 10000} & 52.32 & 56.83 & 63.58 & 63.45& 59.05 & 76.16 & 77.91 & 73.51\\
\textbf{\ourname-BERT 12000} & 52.34 & 56.84 & 63.6 & 63.62&  59.25 & 76.73 & 78.22 & 73.96\\
\textbf{\ourname-BERT 14000} & 52.32 & 56.82 & 63.59 & 63.52& 59.5 & 76.68 & 78.49 & 73.88\\
\textbf{\ourname-BERT 16000} & 52.3 & 56.81 & 63.6 & 63.33 &  58.96 & 76.18 & 77.6 & 73.4\\
\textbf{\ourname-BERT 18000} & 52.33 & 56.84 & 63.58 & 63.65& 59.47 & 76.11 & 78.51 & 73.66\\

% \textbf{\ourname-BERT best(10000)} & 53.06 & 62.32 & 69.88 &63.57&  &&&\\
\textbf{\ournameplus-BERT} & - & - & - &-&  &&&\\
	
\hline

\end{tabular} 



==> tables/llm_main_table.tex <==


\begin{tabular}{l|llll|llll}
\hline
\noalign{\vskip 0.05cm}
&\multicolumn{4}{c}{\textbf{mini-SDv2}} & \multicolumn{4}{c}{\textbf{mini-NQ}}\\
% \textbf{Model} &  \multicolumn{1}{c}{\textbf{Val}} & \multicolumn{1}{c}{\textbf{Test} }& \multicolumn{2}{c}{\textbf{Val}}& \multicolumn{1}{c}{\textbf{Test}}\\
\noalign{\vskip 0.05cm}
\cline{2-9}
\noalign{\vskip 0.05cm}
\textbf{} & \textbf{EM} & \textbf{P} & \textbf{R} &\textbf{F1}& \textbf{EM} & \textbf{P} & \textbf{R} &\textbf{F1} \\
\noalign{\vskip 0.05cm}
\hline
\noalign{\vskip 0.05cm}
% FLAN-T5-XXL&74.79 & 83.71 & 83.74 & 82.48&&&&\\
LLaMA-2-70b-chat& 0.24 & 7.20 & 52.70 & 11.34    & 28.07 & 43.20 & \textbf{79.21} & 46.47\\
text-davinci-003 & 52.37 & 56.86 & 63.58& 58.44 &52.24 & 69.96 & 77.50 & 69.44\\
ChatGPT &	30.89 & 40.53 & \textbf{68.54} & 44.95  &57.53 & 74.15 & 75.81 & 71.54\\
\textbf{Oracle} & 58.61 & 64.04 & 77.98 & 66.20& 64.02 & 80.54 & 87.97 & 79.21\\
\noalign{\vskip 0.05cm}
\hline  
\noalign{\vskip 0.05cm}
MV & 26.95 & 34.23 & 61.22 & 37.75 & 46.07 & 62.56 & 77.66 & 62.43\\
WV  & 52.37 & 56.86 & 63.58 & 58.44 & 57.53 & 74.15 & 75.81 & 71.54\\
PageRank & & & &37.31 & & & &68.53\\
OLA & & & &56.08 & & & &\\

% MLA& & & & & & & &\\
% RANK& & & & & & & &\\
% MCB & & & & & & & &\\
% apriori & & & & & & & &\\
\noalign{\vskip 0.05cm}
\hline
\noalign{\vskip 0.05cm}
% FT-BERT 10 & 27.22 & 28.20 & 30.13 & 28.47& 3.92 & 11.05 & 18.49 & 11.23\\
% \textbf{\ourname-BERT 10} & 51.83 & 56.36 & \textbf{63.74} & \underline{61.78}& 56.19 & 73.66 & 74.22 & 70.41\\

%FT-BERT 300 & 47.45 & 47.86 & 48.67 & 47.96& 24.15 & 29.37 & 29.64 & 27.4\\
%\textbf{\ourname-BERT 300}  & 52.35 & 56.85 & 63.59 & 63.63&57.93 & 74.87 & 75.85 & \underline{71.91}\\
% FT-BERT 600 & 42.41 & 43.15 & 44.51 & 43.22& 32.18 & 38.83 & 39.53 & 36.55 \\
FT-BERT & 46.80 & 47.70 & 48.86 & 47.68& 36.52 & 42.81 & 43.46 & 40.60\\
\textbf{\ourname-BERT} & \textbf{57.74} & \textbf{62.22} & 68.45 & \textbf{63.71}&  \textbf{58.45} & \textbf{75.99} & 77.75 & \textbf{73.37}\\

\textbf{\ournameplus-BERT } & 52.12 & 52.74 & 53.47 & 52.68 &  46.61 & 55.08 & 54.63 & 52.49\\
% \textbf{\ournameplus-BERT 1k} & \textbf{55.41} & 56.22 & 57.30 & 56.21 &  52.79 & 64.20 & 61.78 & 60.9\\
	
\hline

\end{tabular} 






% LLaMA-2-70b& 0.15 & 6.55  & 54.00 & 10.50&5.37&13.13&49.15&17.46\\
% Davinci-003& 47.78 & 56.87 & 64.78& 58.18&24.02&35.36&42.38&36.04\\
% ChatGPT &	29.28 &	39.80  & 70.28& 44.22&32.24&43.83&49.29&43.83\\
% \textbf{Oracle} & 53.94 & 63.86 & 79.34 &65.92& 38.19 &51.93&64.43&52.67\\
% \textbf{\ourname-BERT 10000} & 53.01 & 62.21 & 69.81 &63.47& 31.94 &43.82&48.46&43.87\\

==> tables/main_merged_table.tex <==


\begin{tabular}{l|cccc||l|cc}
\hline \hline

% \noalign{\vskip 0.04cm}

% \rowfont{\normalsize}%

\multicolumn{5}{c||}{ {Textual Question Answering}} & \multicolumn{3}{c}{ {Visual Question Answering}} \\

% \noalign{\vskip 0.04cm}
 \hline \hline
 
\multirow{2}{*}{\textbf{Model}}&\multicolumn{2}{c}{\textbf{Mini-SDv2}} & \multicolumn{2}{c||}{\textbf{Mini-NQ}} & \multirow{2}{*}{\textbf{Model}} &\textbf{Mini-GQA} & \textbf{Mini-Viz}\\
% \textbf{Model} &  \multicolumn{1}{c}{\textbf{Val}} & \multicolumn{1}{c}{\textbf{Test} }& \multicolumn{2}{c}{\textbf{Val}}& \multicolumn{1}{c}{\textbf{Test}}\\
\noalign{\vskip 0.02cm}
\cline{2-5}\cline{7-8}
\noalign{\vskip 0.02cm}
 & \textbf{EM} &\textbf{F1}& \textbf{EM} & \textbf{F1} & &\textbf{Acc} & \textbf{Acc} \\
\noalign{\vskip 0.02cm}
\hline
\noalign{\vskip 0.02cm}
% FLAN-T5-XXL&74.79 & 83.71 & 83.74 & 82.48&&&&\\
LLaMA-2-70b-chat & 0.24  & 11.34    & 28.07 &  46.47 & ALBEF& \underline{50.60} & \underline{21.28}\\
text-davinci-003 & \underline{52.37}  & \underline{58.44} & 52.24 &  69.44 & BLIP & 48.08 &20.80\\
ChatGPT &	30.89  & 44.95  & \underline{57.53} &  \underline{71.54} & VLMo &	48.21 &19.77 \\
\textbf{Oracle} & 58.61  & 66.20& 64.02 &  79.21 & \textbf{Oracle} &  65.03 & - \\
\noalign{\vskip 0.02cm}
\hline  
\noalign{\vskip 0.02cm}
MV & 26.95 &  37.75 & 46.07  & 62.43 & MV & 51.05&21.47\\
WV  & 52.37 &  58.44 & 57.53 & 71.54 & WV  & 52.10&19.43\\
PageRank & 25.39 &37.31 & 51.76 &68.53 & PageRank &51.47&21.66 \\
OLA & 47.90 &55.59 & 54.70 & 70.05 & OLA &48.65&20.32\\
 PairRanker  & 57.28 &  63.33 & 57.96 &72.21 &  PairRanker &52.05 & 22.42\\
(0-shot) LLM-Blender & 4.90 &21.20 &1.03 &25.06 & (0-shot) LLM-Blender&0.0 &0.0 \\
% GENfuser(pairrank) & 71.13 &82.41 &62.06 &76.25 & LLM-Blender&50.10 &- \\

% GENfuser (InfoSel) & 70.96 &82.06& 61.43&76.0 & LLM-Blender& &- \\
% MLA& & & & & & & &\\
% RANK& & & & & & & &\\
% MCB & & & & & & & &\\
% apriori & & & & & & & &\\
\noalign{\vskip 0.02cm}
\hline
\noalign{\vskip 0.02cm}
% FT-BERT 10 & 27.22 & 28.20 & 30.13 & 28.47& 3.92 & 11.05 & 18.49 & 11.23\\
% \textbf{\ourname-TT 10} & 51.83 & 56.36 & \textbf{63.74} & \underline{61.78}& 56.19 & 73.66 & 74.22 & 70.41\\

%FT-BERT 300 & 47.45 & 47.86 & 48.67 & 47.96& 24.15 & 29.37 & 29.64 & 27.4\\
%\textbf{\ourname-TT 300}  & 52.35 & 56.85 & 63.59 & 63.63&57.93 & 74.87 & 75.85 & \underline{71.91}\\
% FT-BERT 600 & 42.41 & 43.15 & 44.51 & 43.22& 32.18 & 38.83 & 39.53 & 36.55 \\
FT-TT & 46.80 & 47.68& 36.52  & 40.60 & FT-MT&50.48& 51.76 \\
\textbf{\ourname-TT (ours)} & \textbf{57.74}  & \textbf{63.63}&  \textbf{58.45} & \textbf{73.37} & \textbf{\ourname-MT (ours)} &\textbf{55.16}&23.16\\

% \textbf{\ournameplus-TT } & 52.12 & 52.68 &  46.61 & 52.49\\
\textbf{\ournameplus-TT (ours)} &  49.09  & 49.85 & 48.16 & 53.70 &  \textbf{\ournameplus-MT (ours)} &52.54&\textbf{52.91}\\
% \textbf{\ournameplus-TT 1k} & \textbf{55.41} & 56.22 & 57.30 & 56.21 &  52.79 & 64.20 & 61.78 & 60.9\\
\noalign{\vskip 0.02cm}	
\hline

\end{tabular} 

% \end{table*}






% LLaMA-2-70b& 0.15 & 6.55  & 54.00 & 10.50&5.37&13.13&49.15&17.46\\
% Davinci-003& 47.78 & 56.87 & 64.78& 58.18&24.02&35.36&42.38&36.04\\
% ChatGPT &	29.28 &	39.80  & 70.28& 44.22&32.24&43.83&49.29&43.83\\
% \textbf{Oracle} & 53.94 & 63.86 & 79.34 &65.92& 38.19 &51.93&64.43&52.67\\
% \textbf{\ourname-TT 10000} & 53.01 & 62.21 & 69.81 &63.47& 31.94 &43.82&48.46&43.87\\

==> tables/multimodal_fusion_table.tex <==
\begin{table*}[h]
\centering
\footnotesize

\begin{tabular}{lcc}
\hline
\textbf{Method} &  & \textbf{Mini-GQA} &\textbf{Mini-Viz} \\
\hline
PairRanker(Q+A) &52.05 & 22.42 \\
% (0-shot) LLM-Blender(Q+A) & 0.0& 0.0\\
\hline
\noalign{\vskip 0.02cm}
\ourname-MT(V)  & 50.56& 20.79 \\
\ourname-MT(Q)  &51.11 & 21.21 \\
\ourname-MT(V+Q)  &50.83 &  20.06\\
\ourname-MT(V+A) &52.38 & 22.66 \\
\ourname-MT(Q+A)  & 54.76&22.89 \\
% \textbf{MC-Q} & 62.11&48. & & \\
\textbf{\ourname-MT(V+Q+A)} &\textbf{55.16}&\textbf{23.16} \\
% \textbf{upbound(FT)} & & &&\\	
\hline

\end{tabular}
\caption{\label{tab:ablation} Accuracy of \textbf{\ourname}-MT models when using different input information for training compared to baseline models. V, Q, and A represent visual, question, and answer information respectively.}
\end{table*}


==> tables/table_main_onedigit.tex <==
\begin{tabular}{l|l|l|ll|l}
\hline
&\multicolumn{2}{c}{\textbf{GQA}} & \multicolumn{3}{c}{\textbf{VizWiz}}\\
\textbf{Model} &  \multicolumn{1}{c}{\textbf{Val}} & \multicolumn{1}{c}{\textbf{Test} }& \multicolumn{2}{c}{\textbf{Val}}& \multicolumn{1}{c}{\textbf{Test}}\\

\cline{2-6}
\textbf{} & \textbf{Acc} & \textbf{Acc} & \textbf{Acc} &\textbf{F1}& \textbf{Acc} \\
\hline

ALBEF&\textbf{54.8}&\textbf{50.6} &21.9&18.8&\textbf{21.3}\\
BLIP& 53.0 & 48.1 &  \textbf{22.6}&19.6&20.8\\
VLMo &	54.0 &	48.2 &22.0&18.0&19.8\\

\textbf{Oracle} & 70.3 & 65.0 & 28.8 &28.1&- \\
\hline
MV &55.9 & 51.1&23.5&2.12&21.5\\
WV  &56.5 & 52.1&23.8&20.6&19.4\\

% Q-Cluster  &56.10 & 51.18&&\\
% QI-Cluster  & 56.38& 51.20&&\\
\ourname-MLP &57.9&52.4&22.7&18.8&21.1\\
% $Selector_s$&58.21 &47.52&& \\

\hline


FT-MT&68.9 & 50.5&\textbf{46.1} &0.0 & \textbf{32.9}\\%$\frac{0}{0}$
\textbf{\ourname-MT} &\textbf{63.0} &\textbf{55.2}&\textbf{25.2}&21.4&\textbf{23.3}\\

\ourname-MT$^2$ &63.0&55.3&55.6&26.6&42.1\\
	
\hline

\end{tabular} 

==> tables/table_main_twodigits.tex <==
\begin{tabular}{l|l|l|ll|l}
\hline
&\multicolumn{2}{c}{\textbf{mini-GQA}} & \multicolumn{3}{c}{\textbf{mini-Viz}}\\
\textbf{Model} &  \multicolumn{1}{c}{\textbf{Val}} & \multicolumn{1}{c}{\textbf{Test} }& \multicolumn{2}{c}{\textbf{Val}}& \multicolumn{1}{c}{\textbf{Test}}\\

\cline{2-6}
\textbf{} & \textbf{Acc} & \textbf{Acc} & \textbf{Acc} &\textbf{F1}& \textbf{Acc} \\
\hline

ALBEF&54.82&50.60 &21.92&20.51&21.28\\
BLIP& 52.94 & 48.08 &22.64&20.08&20.80\\
VLMo &	54.00 &	48.21 &21.95&20.10&19.77\\
\textbf{Oracle} & 70.30 & 65.03 & 28.76&24.87&- \\
\hline
MV &55.85 & 51.05&23.64&21.48&21.47\\
WV  &56.45 & 52.10&23.82&21.59&19.43\\
PageRank &56.30&51.47&24.72&&21.66\\
OLA &54.81&48.65&23.56&&20.32 \\
% Q-Cluster  &56.10 & 51.18&&\\
% QI-Cluster  & 56.38& 51.20&&\\
% \ourname-MLP &57.87&52.35&22.68&18.75&21.12\\
% $Selector_s$&58.21 &47.52&& \\
\hline
FT-MT&68.86 & 50.48& 51.71&20.66& 51.76\\%$\frac{0}{0}$
\textbf{\ourname-MT} &63.00 &\textbf{55.16}&25.13&22.60&23.16\\

\textbf{\ournameplus-MT} &\textbf{70.06}&52.54&\textbf{55.92}&\textbf{32.18}&\textbf{52.91}\\
% \textbf{\ournameplus-MT} &69.40&50.65&56.44&33.57&\textbf{53.69}\\
	
\hline

\end{tabular} 
